A Dictionary Based Approach for Removing Out-of-Focus Blur

The field of image deblurring has seen tremendous progress with the rise of deep learning models. These models, albeit efficient, are computationally expensive and energy consuming. Dictionary based learning approaches have shown promising results in image denoising and Single Image Super-Resolution. We propose an extension of the Rapid and Accurate Image Super-Resolution (RAISR) algorithm introduced by Isidoro, Romano and Milanfar for the task of out-of-focus blur removal. We define a sharpness quality measure which aligns well with the perceptual quality of an image. A metric based blending strategy based on asset allocation management is also proposed. Our method demonstrates an average increase of approximately 13% (PSNR) and 10% (SSIM) compared to popular deblurring methods. Furthermore, our blending scheme curtails ringing artefacts post restoration.

==> name.tex <==
\begin{figure}[htbp]
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face.png}
        \caption{Original Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_blurred.png}
        \caption{Degraded Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_restormer.png}
        \caption{Restormer Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_ifan.png}
        \caption{IFAN Image}
    \end{subfigure}
    
    \medskip % add some vertical space between the rows
    
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_L.png}
        \caption{Landweber Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_NAL.png}
        \caption{NAL Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_PCL.png}
        \caption{PCL Image}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\linewidth]{res_images/face_RAID.png}
        \caption{Ours}
    \end{subfigure}
    
    \caption{Comparison}
\end{figure}


\begin{figure}[hbt!]

    \begin{subfigure}{0.450\linewidth}
      \includegraphics[width=\linewidth]{Blended_Iteration1.png}
      \caption{Blended Image after 1 Iteration}
      \label{fig:iter1_blend}
    \end{subfigure}\hfill % <-- "\hfill"
    \begin{subfigure}{0.450\linewidth}
      \includegraphics[width=\linewidth]{Blended_Iteration2.png}
      \caption{Blended Image after 2 Iteration}
      \label{fig:iter2_blend}
    \end{subfigure}
    
    \medskip % create some *vertical* separation between the graphs
    \begin{subfigure}{0.450\linewidth}
      \includegraphics[width=\linewidth]{Blended_Iteration4.png}
      \caption{Blended Image after 4 Iterations}
      \label{fig:iter4_blend}
    \end{subfigure}\hfill % <-- "\hfill"
    \begin{subfigure}{0.450\linewidth}
      \includegraphics[width=\linewidth]{Blended_Iteration3.png}
      \caption{Blended Image after 3 Iterations}
      \label{fig:iter3_blend}
    \end{subfigure}

    \caption{Blended Images}
    \label{fig:blended_images}
\end{figure}


\begin{table}[htbp]
\tiny
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Patch Size} & \textbf{13} $\times$ \textbf{13} & \textbf{15} $\times$ \textbf{15} & \textbf{21} $\times$ \textbf{21} & \textbf{25} $\times$ \textbf{25} \\ \midrule
\textbf{PSNR (dB)}  & 37.519      & 37.599      & 39.148      & 39.607      \\
\textbf{SSIM}       & 0.960        & 0.961       & 0.967       & 0.969       \\ \bottomrule
\end{tabular}%
}
\caption{Effect of patch size on image quality}
\label{tab:patch_size}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BLENDING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For each image, we calculate metric $Q$ denoted by $Q_1$, $Q_2, \ldots, Q_n$, which we arrange in an ascending order of their magnitudes. We initialize our blending strategy by applying equal weighting to all images $P_i$, where $i \in [1, n]$.  

\begin{equation}
   % I_B = \frac{1}{n}P_1 + \frac{1}{n}P_2 + \ldots + \frac{1}{n}P_n
   I_B = \alpha_1P_1 + \alpha_2P_2 + \ldots + \alpha_nP_n
    \label{eq:equal_weights}
\end{equation}
We represent the weighting coefficients as $\alpha_i$ = $\frac{1}{n}$, where $i \in [1, n]$. 

The first step consists of updating the coefficients of the images with the minimum and maximum values of $Q$, i.e. $\alpha_1$ and $\alpha_n$, by measuring the increase factor $k$ between the two images, subtracting it from $\alpha_1$ and adding it to $\alpha_n$, thereby concluding step 1 of the first iteration.
We now have:
\begin{equation}
    I_B = (\alpha_1 - k)P_1 + \alpha_2P_2 + \ldots + (\alpha_n + k)P_n
    \label{eq:iter1}
\end{equation}
Repeating the aforementioned procedure a second time, we get:
\begin{equation}
    I_B = (\alpha_1 - k)P_1 + (\alpha_2 - k')P_2 + \ldots + (\alpha_n + k + k')P_n
    \label{eq:iter2}
\end{equation}
where $k'$ is the increase factor between images $\alpha_2$ and $\alpha_n$.

Similarly, repeating this until we reach the stage when the coefficient associated with $P_{n-1}$ has the minimum value of $Q$, we get:
\begin{multline}
        I_B = (\alpha_1 - k)P_1 + (\alpha_2 - k')P_2 + 
    \ldots + (\alpha_{n-1} - k^{(n-1)'})P_{n-1} + \\ (\alpha_n + k' + k'' + \ldots + k^{(n-1)'})P_n
    \label{eq:final_it1}
\end{multline}
This concludes iteration 1.

As the weighting coefficient associated with $P_n$ has reached the maximum value, we shall denote it using the symbol $\theta^{(1)}_n$. The terms $(\alpha_i - k^{(i-1)'})$ can be represented as $\gamma^{(1)}_{\{i\}}$, where $i \in [1, n]$. We can rewrite equation~(\ref{eq:final_it1}) as:
\begin{equation}
    I_B = \gamma^{(1)}_{\{1\}}P_1 + \gamma^{(1)}_{\{2\}} + \ldots + \gamma^{(1)}_{\{n-1\}}P_{n-1} +
    \theta^{(1)}_{n}P_n. 
    \label{eq:rewrite_eq_1}
\end{equation}
For the second iteration, we will work only with images associated with coefficients ranging from $\gamma^{(1)}_{\{1\}}$ to $\gamma^{(1)}_{\{n-1\}}$, i.e. $P_1$ to $P_{n-1}$. Following suit the iterative process mentioned above, we calculate the increase factor between values of $Q$ associated with the images having the minimum and maximum values, i.e. images $P_1$ and $P_{n-1}$ respectively, denoted by $l$ and subtracting it from $P_1$ and adding to $P_{n-1}$. We get:
\begin{equation}
    I_B = (\gamma^{(1)}_{\{1\}} - l)P_1 + \gamma^{(1)}_{\{2\}}P_2 + \ldots + (\gamma^{(1)}_{\{n-1\}} + l)P_{n-1} + \theta^{(1)}_{n}P_n.
    \label{eq:second_iteration}
\end{equation}
Likewise, repeating the aforementioned step for all weighting coefficients associated with $P_i$, where $i \in [2, n-1]$, we get:
\begin{multline}
    I_B = (\gamma^{(1)}_{\{1\}} - l)P_1 + (\gamma^{(1)}_{\{2\}} - l')P_2 + \ldots + \\ (\gamma^{(1)}_{\{n-1\}} + l' + l'' + \ldots + l^{(n-2)'})P_{n-1} + \theta_{n}^{(1)}P_n
    \label{eq:second_iteration_1}
\end{multline}
Rewriting equation~(\ref{eq:second_iteration_1}) in a similar fashion to ~(\ref{eq:rewrite_eq_1}), we get:
\begin{multline}
    I_B = \gamma_{\{1\}}^{(2)}P_1 + \gamma_{\{2\}}^{(2)}P_2 + \ldots + \gamma_{\{n-2\}}^{(2)}P_{n-2} + \\ \theta_{n-1}^{(2)}P_{n-1} + \theta_{n}^{(1)}P_n
    \label{eq:second_iteration_end}
\end{multline}
Performing this iterative process a third time, we get:
\begin{multline}
    I_B = \gamma_{\{1\}}^{(3)}P_1 + \gamma_{\{2\}}^{(3)}P_2 + \ldots + \\ \gamma_{\{n-3\}}^{(3)}P_{n-3} + \theta_{n-2}^{(3)}P_{n-2} + \theta_{n-1}^{(2)}P_{n-1} + \theta_{n}^{(1)}P_n
\end{multline}
This iterative process is continued till we reach the point when metric $Q$ value for $P_2$ is the maximum value and $P_1$ is the minimum value. We get:
\begin{multline}
    I_B = \gamma_{\{1\}}^{(n)}P_1 + \theta_2^{(n-1)}P_2 + \theta_3^{(n-2)}P_3 + \ldots + \theta^{(2)}_{n-1}P_{n-1} + \theta^{(1)}_{n}P_n
    \label{eq:final_eq_1}
\end{multline}
Finally, we get:
\begin{equation}
     I_B = \theta_{1}^{(n)}P_1 + \theta_2^{(n-1)}P_2 + \theta_3^{(n-2)}P_3 + \ldots + \theta^{(2)}_{n-1}P_{n-1} + \theta^{(1)}_{n}P_n
    \label{eq:final_eq_2}
\end{equation}


\begin{table}[htbp]
\tiny
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}clrr@{}}
\toprule
\textbf{Dataset} & \multicolumn{1}{c}{\textbf{Algorithm}} & \multicolumn{1}{c}{\textbf{PSNR (dB)}} & \multicolumn{1}{c}{\textbf{SSIM}} \\ \midrule
                                 & IFAN \cite{lee2021iterative}                                & 23.100                         & 0.653                         \\
                                 & Restormer \cite{zamir2022restormer}                           & 24.566                         & 0.723                         \\
                                 & NBDNet \cite{chen2021learning}                              & 27.280                         & 0.754                         \\
                                 & Landweber \cite{wang2023reverse}                        & 26.263                         & 0.757                         \\
                                 & \cellcolor[HTML]{C0C0C0}NA Landweber & \cellcolor[HTML]{C0C0C0}26.291 & \cellcolor[HTML]{C0C0C0}0.758 \\
                                 & \cellcolor[HTML]{C0C0C0}PC Landweber & \cellcolor[HTML]{C0C0C0}27.732 & \cellcolor[HTML]{C0C0C0}0.820  \\
\multirow{-7}{*}{\textbf{Set14}} & \textbf{Ours}                        & \textit{\textbf{29.287}}       & \textit{\textbf{0.847}}       \\ \midrule
                                 & IFAN                                 & 25.409                         & 0.789                         \\
                                 & Restormer                            & 26.645                         & 0.823                         \\
                                 & NBDNet                               & 31.036                         & 0.869                         \\
                                 & Landweber                            & 29.011                         & 0.849                         \\
                                 & \cellcolor[HTML]{C0C0C0}NA Landweber & \cellcolor[HTML]{C0C0C0}30.019 & \cellcolor[HTML]{C0C0C0}0.867 \\
                                 & \cellcolor[HTML]{C0C0C0}PC Landweber & \cellcolor[HTML]{C0C0C0}30.715 & \cellcolor[HTML]{C0C0C0}0.890 \\
\multirow{-7}{*}{\textbf{Set5}}  & \textbf{Ours}                        & \textit{\textbf{31.999}}       & \textit{\textbf{0.900}}       \\ \bottomrule
\end{tabular}%
}
\caption{Quantitative Comparison with set14 and set5}
\label{tab:results_table}
\end{table}

%We select \textbf{criterion 2} from the list of termination criteria as $Q(I_B^{2}) <  Q(I_B^{1})$ to stop the consecutive application of our algorithm. %The calculated $Q$ for $I_B^{2}$ is 5.2771. Performing the mechanism a third time produces a blended image with a $Q$ value of 5.2688.

%% Principal gradient 

P - 4.2 (ICIP) Restoration + ENhanceme
P2 = 4.1 
Deblurring, Restoration, Optical Blur, LEarned Filter, Sharpness
